Relational Graph Convolutional Networks: A Closer Look

In this paper, we describe a reproduction of the Relational Graph Convolutional Network (RGCN). Using our reproduction, we explain the intuition behind the model. Our reproduction results empirically validate the correctness of our implementations using benchmark Knowledge Graph datasets on node classification and link prediction tasks. Our explanation provides a friendly understanding of the different components of the RGCN for both users and researchers extending the RGCN approach. Furthermore, we introduce two new configurations of the RGCN that are more parameter efficient. The code and datasets are available at https://github.com/thiviyanT/torch-rgcn.

==> images/nn.tex <==
 \def\layersep{4.9}
 \def\actsep{2.1}
\begin{tikzpicture}[shorten >=1pt,->,draw=black!50, node distance=\layersep, scale=0.4]
    \tikzstyle{every pin edge}=[<-,shorten <=1pt]
    \tikzstyle{neuron}=[circle,draw=black,thick,minimum size=24pt,inner sep=1pt]
    \tikzstyle{box}=[rectangle,rounded corners,fill=black!5,draw=black!50,thick,minimum size=21pt,inner sep=1.5pt]
    \tikzstyle{input neuron}=[neuron];
    \tikzstyle{output neuron}=[neuron];
    \tikzstyle{hidden neuron}=[neuron];

    \foreach \name / \y in {1,2,3}
        \node[input neuron] (I-\name) at (-\layersep,-3*\y+6) {$x_{\y}$};
    
    \foreach \name / \y in {1,...,4}
        \path
            node[hidden neuron] (H-\name) at (\layersep,-3*\y+7.5) {$\Phi^{(1)}_{\y}$};
    
    \foreach \source in {1,2,3}
        \foreach \dest in {1,...,4}
            \path (I-\source) edge (H-\dest);

    \node[box] (G-1) at (0,0) {$x\mapsto W^{(1)}x+b^{(1)}$};
    
    \foreach \name / \y in {1,...,4}
        \path
            node[hidden neuron] (Ha-\name) at (\layersep+2*\actsep,-3*\y+7.5) {$\bar{\Phi}^{(1)}_{\y}$};

    \foreach \source in {1,2,3,4}
        \path (H-\source) edge (Ha-\source);
        
    \node[box] (G-2) at (\layersep+\actsep,0) {$\varrho$};
    
    \foreach \name / \y in {1,...,6}
        \path
            node[hidden neuron] (L-\name) at (3*\layersep+2*\actsep,-3*\y+10.5) {$\Phi^{(2)}_{\y}$};
    
    \foreach \source in {1,...,4}
        \foreach \dest in {1,...,6}
            \path (Ha-\source) edge (L-\dest);

    \node[box] (G-3) at (2*\layersep+2*\actsep,0) {$x\mapsto W^{(2)}x+b^{(2)}$};
        
    \foreach \name / \y in {1,...,6}
        \path
            node[hidden neuron] (La-\name) at (3*\layersep+4*\actsep,-3*\y+10.5) {$\bar{\Phi}^{(2)}_{\y}$};

    \foreach \source in {1,...,6}
        \path (L-\source) edge (La-\source);
            
    \node[box] (G-4) at (3*\layersep+3*\actsep,0) {$\varrho$};
        
    \node[output neuron] (out) at (5*\layersep+4*\actsep,0){$\Phi_\arch$};

    \foreach \source in {1,...,6}
        \path (La-\source) edge (out);

    \node[box] (G-5) at (4*\layersep+4*\actsep,0) {$x\mapsto W^{(3)}x+b^{(3)}$};
\end{tikzpicture}
